Preserving Derivative Information while Transforming Neuronal Curves

The international neuroscience community is building the first comprehensive atlases of brain cell types to understand how the brain functions from a higher resolution, and more integrated perspective than ever before. In order to build these atlases, subsets of neurons (e.g. serotonergic neurons, prefrontal cortical neurons etc.) are traced in individual brain samples by placing points along dendrites and axons. Then, the traces are mapped to common coordinate systems by transforming the positions of their points, which neglects how the transformation bends the line segments in between. In this work, we apply the theory of jets to describe how to preserve derivatives of neuron traces up to any order. We provide a framework to compute possible error introduced by standard mapping methods, which involves the Jacobian of the mapping transformation. We show how our first order method improves mapping accuracy in both simulated and real neuron traces under random diffeomorphisms. Our method is freely available in our open-source Python package brainlit.

==> 4-downsample.tex <==
Heretofore, we were focused on curves that were known only by a discrete sampling of knots. In this section, we will examine a couple examples where the underlying curve $c$ is smooth, and known. The positions and derivatives of the curve are then discretely sampled. It is natural to assume that the first order mapping method should be more accurate in this setting, since it uses derivative information that the zeroth order method does not. For interpolation, derivative information has proven useful in previous research comparing Lagrange interpolation to Hermite interpolation \cite{devia2019comparison}. However, the only well-known theoretical advantages of using derivative information is in the limiting behavior at the knots \cite{kincaid2009numerical}. In the two examples shown in Figure \ref{fig:toy}g-j, the first order method matches ground truth better than the zeroth order method.


